$\texttt{matryoshka}$: Halo Model Emulator for the Galaxy Power Spectrum

We present $\texttt{matryoshka}$, a suite of neural network based emulators and accompanying Python package that have been developed with the goal of producing fast and accurate predictions of the nonlinear galaxy power spectrum. The suite of emulators consists of four linear component emulators, from which fast linear predictions of the power spectrum can be made, allowing all nonlinearities to be included in predictions from a nonlinear boost component emulator. The linear component emulators includes an emulator for the matter transfer function that produces predictions in $\sim 0.0004 \ \mathrm{s}$, with an error of $<0.08\%$ (at $1\sigma$ level) on scales $10^{-4} \ h \ \mathrm{Mpc}^{-1}<k<10^1 \ h \ \mathrm{Mpc}^{-1}$. In this paper we demonstrate $\texttt{matryoshka}$ by training the nonlinear boost component emulator with analytic training data calculated with HALOFIT, that has been designed to replicate training data that would be generated using numerical simulations. Combining all the component emulator predictions we achieve an accuracy of $< 0.75\%$ (at $1\sigma$ level) when predicting the real space nonlinear galaxy power spectrum on scales $0.0025 \ h \ \mathrm{Mpc}^{-1}<k<1 \ h \ \mathrm{Mpc}^{-1}$. We use $\texttt{matryoshka}$ to investigate the impact of the analysis setup on cosmological constraints by conducting several full shape analyses of the real space galaxy power spectrum. Specifically we investigate the impact of the minimum scale (or $k_\mathrm{max}$), finding an improvement of $\sim 1.8\times$ in the constraint on $\sigma_8$ by pushing $k_\mathrm{max}$ from $k_\mathrm{max}=0.25 \ h \ \mathrm{Mpc}^{-1}$ to $k_\mathrm{max}=0.85 \ h \ \mathrm{Mpc}^{-1}$, highlighting the potential gains when using clustering emulators such as $\texttt{matryoshka}$ in cosmological analyses.

==> sections/galhalo.tex <==
A key quantity for calculating predictions for galaxy clustering in the halo model framework is the occupation number $N(M)$, this occupation number is given by a \textit{halo occupation distribution} (HOD) model. A HOD model is a probabilistic model that described the expected number of galaxies $N$ of a given type with a host halo of $M$. HOD models generally have separate terms that describe the occupation of central and satellite galaxies separately, such that the total expected occupation is given by $N(M) = N_{\text{cen.}}(M)+N_{\text{sat.}}(M)$.

For this work we use a simplification of the extensively used Zheng HOD model, where $N_\text{cen.}(M)$ is modelled as a simple step function
\begin{equation}
    N_\text{cen.}(M) = 
    \begin{cases}
      0 & \text{if}\ M<M_{min}, \\
      1 & \text{if}\ M \geq M_{min},
    \end{cases}
    \label{eq:3par_Ncen}
\end{equation}
where $M_{min}$ simply controls a minimum mass for a halo to host a central galaxy. And $N_\text{sat.}$ is modelled as a power law
\begin{equation}
    N_\text{sat.}(M) = \left( \frac{M}{M_1} \right)^{\alpha},
    \label{eq:3par_Nsat}
\end{equation}
where $M_1$ is the minimum mass for a halo to host at least one satellite in addition to the central galaxy, and $\alpha$ describes how quickly the number of galaxies increases with halo mass (can be thought of as a rough proxy for galaxy formation efficiency).

Our model also modulates the satellite occupation with the central occupation, such that a halo can only host a satellite galaxy if it already hosts a central

\begin{center}
\begin{equation}
    N(M) = N_\text{cen.}(M)\left[1+N_\text{sat.}(M)\right].
\end{equation}
\end{center}

\begin{figure}
	\includegraphics[width=\columnwidth]{plots/3param_cenmod.png}
    \caption{The mean halo occupation number as a function of halo mass for the HOD model used for this work. The dashed line represents the central occupation, the dotted line represents satellite occupation, and the solid line represents the total occupation number.}
    \label{fig:hod_model}
\end{figure}
